Complex-valued neural networks for voice anti-spoofing

Current anti-spoofing and audio deepfake detection systems use either magnitude spectrogram-based features (such as CQT or Melspectrograms) or raw audio processed through convolution or sinc-layers. Both methods have drawbacks: magnitude spectrograms discard phase information, which affects audio naturalness, and raw-feature-based models cannot use traditional explainable AI methods. This paper proposes a new approach that combines the benefits of both methods by using complex-valued neural networks to process the complex-valued, CQT frequency-domain representation of the input audio. This method retains phase information and allows for explainable AI methods. Results show that this approach outperforms previous methods on the "In-the-Wild" anti-spoofing dataset and enables interpretation of the results through explainable AI. Ablation studies confirm that the model has learned to use phase information to detect voice spoofing.

==> sections/compl.tex <==
complex-valued neural networks use many of the same building blocks as real-valued ones.
linear layers, convolutions and simple recurrency such as RNN work exactly the same.
attention and recurrency such as GRU require some modifications, since activation functions such as sigmoid, tanh, and softmax cannot be applied directly to complex valued scalars.

==> sections/intro_outline.tex <==
artificial intelligence becomes more powerful
many good and helpful applications
but also many new threats, especially deepfake and spoofs
deepfakes can be misused for fake news, information campagins, slander, fraud.
spoofs can be used to circumvent biometric id systems
thus, the detection of spoofed or faked content becomes every more important.

in the domain of audio and voice, spoofing detection especially important. 
much previous work has been suggested, using machine learning (ML) to learn a binary spoofing classifier from a supervised set of training data.
using ML for audio requires adequate preprocessing
audio and voice are represented as long sequence of scalar values, which cannot be processed by most neural architectures directly.
this is because of long-range dependencies in audio, where usually one second of audio is represented by 16000 single data points or more.

previous voice anti-spoofing have approached this problem in one of two ways.
either they employed spectral preprocessing.
this means the transformed the audio to some magnitude-based spectogram, using the short time fourrier transform (STFT).
this has shown reasonable performance, but has one key disadvantage:
These approaches discard phase information from the spectogram.
given a real-valued time series (such as input audio wav), STFT yields a complex-valued spectogram where the magnitude corresponds to energy and the angle of the complex-valued scalars correpsonds to the phase.
Usually employed spectral features such as CQCC or Mel-Spectogram discard phase information.
However, phase information crucial for audio quality.
In domain of speech-to-text, phase information labrouriously recreated using griffin lim or neural vocoders.
bad phase is very audible, thus we conjecture that it is a very useful feature which is unnecessarily discarded.

Second approach is to design models which process raw audio directly.
This is done by employing stacks of convolutions and sinc-fileters, which are equivalent to band-bass filters.
These models have been shown to be more effective in voice anti-spoofing, but do not afford explainability.
this is because saliency maps require input data with spatial dimensions.

In this work, we present a new approach to voice anti-spoofing which combines the benefit of the previous approaches.
We transform input audio into complex-valued spectogram using STFT, which yields a complex-valued freqency representation.
We process this using complex-valued convoluaiton neural network.

==> tex/original_submission/abstract.tex <==

Current anti-spoofing and audio deepfake detection systems use either magnitude spectrogram-based features (such as CQT or Melspectrograms) or raw audio processed through convolution or sinc-layers. Both methods have drawbacks: magnitude spectrograms discard phase information, which affects audio naturalness, and raw-feature-based models cannot use traditional explainable AI methods.
This paper proposes a new approach that combines the benefits of both methods by using complex-valued neural networks to process the complex-valued, CQT frequency-domain representation of the input audio. This method retains phase information and allows for explainable AI methods.
Results show that this approach outperforms previous methods on the "In-the-Wild" anti-spoofing dataset and enables interpretation of the results through explainable AI.
Ablation studies confirm that the model has learned to use phase information to detect voice spoofing.

==> tex/original_submission/content.tex <==

\section{Introduction}
Artificial Intelligence (AI) is advancing at a rapid pace, and has enabled the development of numerous good and helpful applications that are changing the way we live, work, and interact with each other. However, along with these positive advancements, new threats have emerged, particularly in the form of deepfakes and spoofs.
Deepfakes are computer-generated images, videos, or audio that are created using AI algorithms to manipulate and alter original content. Although deepfakes can be used for harmless fun, they can also be misused for malicious purposes such as creating fake news, information campaigns, slander, or fraud. This is concerning as deepfakes can be highly convincing, making it challenging to distinguish between genuine and fake content.
Spoofing, on the other hand, involves creating a fake or manipulated version of oneself to circumvent biometric identification systems such as facial recognition or fingerprint scanners. This has significant implications, especially in the realm of security, as it can compromise the integrity of identity verification systems.
As a result, the detection of spoofed or faked content is becoming increasingly important. It is crucial to develop effective methods for detecting such misuse of AI in order to ensure that these technologies are used ethically and responsibly.

%One of the two areas that require the application of anti-spoofing the most is voice (the other being video). Many previous studies have utilized machine learning (ML) to develop a binary spoofing classifier from a supervised set of training data. 
Using Machine Learning (ML) for voice anti-spoofing requires adequate preprocessing because 
%audio is represented as a long sequence of scalar values that most neural architectures cannot process directly. This is because
human speech has long-range temporal dependencies, with one second of audio usually represented by $16,000$ single data points or more.
Previous approaches to voice anti-spoofing have taken one of two approaches to audio preprocessing. Some have used spectral preprocessing, transforming the time-domain waveform into a magnitude spectrogram using the short-time Fourier transform (STFT) or similar techniques. This approach has shown good performance but has one key disadvantage: it discards phase information from the spectrogram. This phase information is crucial for audio quality and voice naturalness~\cite{griffin1984signal}, and in the domain of speech-to-text (STT), it is laboriously recreated using Griffin-Lim or neural vocoders~\cite{griffin1984signal, oord2016wavenet, chen2020wavegrad}. As bad phase is very audible\footnote{Audio examples available at \href{https://google.github.io/phase-prediction}{google.github.io/phase-prediction}.}, we argue that it is a useful feature that should not be discarded.

The second approach to voice anti-spoofing is to design models that process raw audio directly,
%. This is accomplished by using stacks of convolutions and sinc-filters that are equivalent to band-pass filters. These models have 
which have been shown to be more effective~\cite{tak2021end, tak2021EndtoEnd, ge2021raw}, but lack transparency because explainable AI methods (XAI) such as saliency maps require input data with spatial dimensions.

In this paper, we propose a new approach to voice anti-spoofing that combines the benefits of both previous approaches. We transform input audio into a complex-valued spectrogram using the constant-Q transform, a technique closely related to the STFT, which yields a complex-valued frequency representation.
This representation is mathematically equivalent to the time-domain representation of the input audio, but more suited to machine-learning algorithms.
We then process this frequency representation using a complex-valued convolutional neural network, which allows us to process all information present in the audio file, without the need to discard the phase.
We demonstrate that our proposed approach outperforms both magnitude spectrogram-based models and raw-feature models. Our approach is conceptually and architecturally simple, which sets it apart from some of the recent state-of-the-art raw models. Moreover, it enables the use of explainable AI techniques.

In summary, our contributions to the field of voice anti-spoofing can be outlined as follows:
\begin{itemize}
\item We emphasize the significance of phase information in the complex Short-Time Fourier Transform (STFT) output, which has been neglected in previous research.
\item Based on this insight, we propose a corresponding complex-valued input feature and neural architecture for jointly processing both magnitude and phase information.
% \item To the best of our knowledge, we are the first to
%\item We employ complex-valued neural networks to jointly process phase and magnitude information using complex-valued spectrograms in the context of voice anti-spoofing.
\item We evaluate our approach and demonstrate its superiority over both magnitude spectrogram-based models and raw-based models.
\end{itemize}
We provide the source code,
%\todo{KB PS ok? -> see comment}
and offer an online web interface where one can test arbitrary input, including YouTube videos, against our model\footnote{To comply with Interspeech's double-blind requirements, the URL will be shared upon acceptance.}.

\section{Previous Work}
% As outlined above, voice anti-spoofing has traditionally used one of two approaches to feature preprocessing.
% There are models which employ magnitude-spectal features such as the constant-Q transform~\cite{brown1991calculation}, log or mel-scaled spectrograms~\cite{stevens1937scale}.
% All of these use the complex-valued STFT of a time-domain audio as foundation, from which they extract the magnitude and discard the phase information.
% Then, the result may be scaled and binned using the mel-scale~\cite{stevens1937scale}, in order to mimic the perception of the human ear.
% The resulting spectogram is then processed using traditional architectures such as convolutions, attention mechanism,  recurrency or transformer blocks~\cite{wang2021Comparative,lavrentyeva_audio_2017,lavrentyeva_stc_2019,afchar2018MesoNet,vaswani2017attention}

% Another approach is to directly process the time-domain, 'raw' audio. Is done using either convolutions directly on the audio file~\cite{chintha2020Recurrent} or stacks of sinc-layers~\cite{ravanelli2018speaker}, which correspond to rectangular band-pass filters.
% Often, in order to avoid phase mismatch between the audio waveform and the sinc wavelets, max-pooling is used~\cite{tak2021EndtoEnd}.
% The result is then processed using stacks of convolutions and gated recurrency (RawNet2)~\cite{tak2021EndtoEnd} or more advanced arechitectures such as spectro-temproal graph attention neural networks (RawGat-ST)~\cite{tak2021end} or differentiable architecture search~\cite{ge2021raw}.

As previously mentioned, voice anti-spoofing traditionally employs one of two feature preprocessing approaches. The first approach involves using magnitude-spectral features like the constant-Q transform (CQT)~\cite{brown1991calculation}, log or mel-scaled spectrograms~\cite{stevens1937scale}. These techniques use the complex-valued STFT of a time-domain audio signal as a foundation, extracting the magnitude and discarding phase information. The result is then squared, scaled, and possibly binned using the mel-scale~\cite{stevens1937scale} to mimic the human ear's perception. Previously suggested voice anti-spoofing architectures have then employed neural components such as convolutions, attention mechanisms, recurrence, or transformer blocks~\cite{wang2021Comparative,lavrentyeva_audio_2017,lavrentyeva_stc_2019,afchar2018MesoNet,vaswani2017attention} to process the resulting spectrogram.
These models have shown good performance, but no longer achieve state of the art.

The second approach involves directly processing the time-domain ``raw'' audio using either neural convolutions on the audio file itself~\cite{chintha2020Recurrent} or stacks of sinc-layers~\cite{ravanelli2018speaker} corresponding to rectangular band-pass filters. 
Max-pooling is often used~\cite{tak2021EndtoEnd} to avoid phase mismatch between the audio waveform and the sinc wavelets. The result is then processed using stacks of convolutions and gated recurrence (RawNet2) \cite{tak2021EndtoEnd}, more advanced architectures like spectro-temporal graph attention neural networks (RawGat-ST) \cite{tak2021end}, or differentiable architecture search~\cite{ge2021raw}.

Although these ``raw'' models have been shown to deliver outstanding performance \cite{tak2021end, tak2021EndtoEnd, ge2021raw}, they lack explainability. This is because existing XAI techniques such as saliency maps~\cite{simonyan2014very} or Smooth Grad~\cite{smilkov2017smoothgrad} are designed for spatially-dimensioned input, while ``raw'' audio is a one-dimensional vector. As a result, it becomes challenging to comprehend and trust the models' judgments.
Among other disadvantages, this impedes the detection of ``learning shortcuts'' \cite{geirhos2020shortcut}, i.e. highly predictive, but artificial correlations between input and target which do not reflect real-world causality. 
Detecting such shortcuts is particularly crucial in voice spoof detection, where they have already been identified \cite{muller2021Speech} and may result in a lack of generalizability to real-world scenarios \cite{muller2022does}. Thus, there is an urgent demand for explainable anti-spoofing models.


\section{Proposed Approach}
% In this section, we introduce our proposed approach and provide background information on the complex-valued frequency representation of audio and its processing by neural networks.

\subsection{Complex-valued CQT spectrograms}
In digital signal processing, an input audio signal $X = [X[0], X[1], \ldots, X[n]]$ is represented in the time domain as a series of scalar values $X[i] \in [-1, 1] \in \mathbb{R}$, which correspond to measurements of air pressure at time $i/s$, where $s$ is the sampling rate (e.g., 16~kHz or 16,000 samples per second). To convert this signal into a frequency representation $Z$, one may use the Short Time Fourier Transform, which is a bijective transform:

\begin{equation}
    Z[t, k] = \sum_{n=0}^{N-1} W[n]X[n+t]e^{-2 \pi i k n N^{-1}}
\end{equation}
Here, $X$ is the time-domain signal, and $W$ is a window such as the Gaussian, Hann, or Hamming window of size $N$. 
The frequency-domain representation $Z$ is a complex-valued, two-dimensional vector, where $t$ is the temporal and $k$ the frequency index. 
Elements in $Z$ are complex-valued scalars, i.e. $Z[t, k] = \alpha e^{i \theta} \in \mathbb{C}$, where $\alpha \in \mathbb{R}$ is the magnitude and $\theta \in [0, 2\pi[$ the phase.

Although $Z$ is better suited for neural processing than the corresponding time-domain representation $X$, it also has its own drawbacks: the uniform time and frequency resolution for all frequency bins $k$ does not align with the non-linearities of the human auditory system~\cite{mceachern1992ear, moore2012introduction}.
To address this issue, we employ the constant Q transform (CQT)~\cite{brown1991calculation, blankertz2001constant} which processes the same number of cycles $Q$ for each frequency and spaces the frequency bins $k$ geometrically (i.e., higher frequencies are farther apart).
Therefore, for high frequencies $k$, CQT employs smaller window sizes $N_k$ (and thus higher time resolution), while for lower frequencies, it employs larger window sizes and thus larger frequency resolution.
Thus, instead of using the STFT, we convert time-domain audio $X$ into a complex-valued CQT spectrogram:
\begin{equation}
    Z_Q[t, k] = \frac{1}{N_k} \sum_{n=0}^{N_k-1} W_k[n] X[n+t] e^{-2 \pi i QnN_k^{-1}}
\end{equation}
Previous work has already shown that magnitude-based CQT is better suited to voice antispoofing than magnitude-based STFT~\cite{todisco2017constant}, which motivates our approach.

Finally, we convert the complex-valued CQT-spectrogram into a log representation by means of the following transformation:
\begin{align}
    \mathbb{C} & \to \mathbb{C}  \\
    |z| e^{i \theta} & \mapsto 
    % \text{max} \left(0, -\frac{z\text{log}_e |z|}{|z|} + c \right )  = 
    \text{max} \left(\epsilon, -\text{log}_e |z| + c\right) \cdot \alpha \cdot e^{i \theta}
    \label{eq:logscale}
\end{align}
To account for the logarithmic perception of sound level by the human ear, we log-scale the magnitude of the complex number while keeping the phase intact.
However, $\text{log}_e |z|$ can be negative, leading to ambiguity, because $\text{log}_e |z| e^{i\theta} = -\text{log}_e |z| e^{i\theta + i\pi}$.
To address this, we apply a lower threshold of $\epsilon > 0$ to ensure that the magnitude remains positive.
Additionally, to ease model training, we introduce trainable parameters $\alpha, c \in \mathbb{R}^{\geq 0}$ to appropriately scale the magnitude.
% We empirically find that suitable initializations are $\alpha=0.15$ and $c = -0.3$.
To summarize, we utilize CQT followed by \cref{eq:logscale} to generate complex-valued CQT log-spectrograms (C-CQT).

% Good test, but already said several times.
% Traditional preprocessing approaches transform $Z$ into a power-spectrogram by mapping the complex values to their absolute values and squaring the result. However, this operation discards the angle of the complex number, which corresponds to the phase information. It is well known from text-to-speech (TTS) research that this phase information is crucial for natural-sounding audio~\cite{griffin1984signal}, which is why we argue to keep $Z$ complex-valued and to consequently employ complex-valued neural networks to make full use of the information available.

\subsection{Complex-valued neural networks}
Complex-valued neural networks (CVNN) are networks where both inputs $X$ and weights $\theta$ are complex numbers $a + ib \in \mathbb{C}$. Apart from that, CVNNs rely on many of the same fundamental components as traditional real-valued ones. For instance, linear layers, convolutions, and simple recurrent networks like RNN operate identically in both types of networks. However, more complex components such as attention and recurrence, such as GRU~\cite{cho2014properties}, need to be adapted, since typical activation functions like \emph{sigmoid}, \emph{tanh}, and \emph{softmax} cannot be applied directly to complex-valued scalars \cite{bassey2021survey}.
For example, the complex \emph{ReLU} function can be implemented as
\begin{equation}
    CReLU(x) = \text{max}(0, \Re(x)) + i \text{max}(0, \Im(x))
\end{equation}
where $\Re$ and $\Im$ denote the real and imaginary parts of a complex number.
In supervised classification, class scores $y$ for $n$ classes can be derived from complex-valued logits $z$ as follows:
\begin{equation}
    \text{softmax}(|z|)_i = \frac{e^{|z_i|}}{\sum_{j=1}^n e^{|z_j|}}
    \label{eq:act}
\end{equation}
Classes with high probability are represented by logits with a large magnitude. These models, like their real counterparts, are trained using gradient descent~\cite{bassey2021survey} through the use of Wirtinger Calculus~\cite{wirtinger1927formalen}.

\subsection{Proposed Architecture}
In order to process complex-valued, frequency-domain audio input, we use a complex convolutional network.
It consists of four blocks of convolutions, where each block is composed of two-dimensional complex convolutions (kernel size $3$, stride $2$ and padding $1$), complex ReLU and complex Batch-Normalisation.
This is followed by linear projection, which consists of three complex-valued linear layers with CReLU activation and Dropout of $40\%$. This is followed by two-dimensional complex time pooling.
The output is a two-class complex vector of shape $(B, 2)$, to which we apply \cref{eq:act} in order to obtain real-valued class scores.
There are two target classes: class $0$, which corresponds to bonafide audio, and class $1$, which corresponds to spoofed audio.
The input frequency-domain audio has shape $B, F, T$ where $B$ is the batch-size, $F$ the number of frequency bins, and $T$ the number of time bins. The convolutional stack outputs a tensor $B, C, L$ where $C$ is the number of output channels and $L$ is the aggregated time.
\Cref{fig:architecture} provides an overview.



\begin{figure}
    \centering
    \includegraphics[width=0.22\textwidth]{res/cvnn.png}
    \caption{Our proposed complex-valued architecture. }
    \label{fig:architecture}
\end{figure}

\section{Evaluation}
\subsection{Datasets}
We are utilizing two datasets for our experiments. The first dataset is the Logical Access (LA) section of the ASVspoof 2019 dataset~\cite{todisco2019asvspoof}. This dataset is widely used in related research~\cite{tak2021end,tak2021EndtoEnd,ge2021raw,wang2021Comparative,lavrentyeva_audio_2017,lavrentyeva_stc_2019,afchar2018MesoNet,vaswani2017attention} and is considered one of the most established anti-spoofing datasets.
It includes audio files that are either genuine human speech recordings (bona-fide) or manipulated/synthesized audio (spoofed). The spoofed audio files are generated using 19 different Text-To-Speech (TTS) synthesis algorithms that are considered a threat to the authenticity of human voice in terms of spoofing detection. Therefore, the spoofed audio files are labeled as ``attacks'' by ASVspoof. The dataset consists of 19 attackers, labeled as A1 to A19, and for each attacker, there are 4914 synthetic audio recordings and 7355 genuine samples.

Furthermore, we utilize the ``In-the-Wild'' (ITW) dataset~\cite{muller2022does}, which comprises $37.9$ hours of audio recordings, either spoofed ($17.2$ hours) or authentic ($20.7$ hours), obtained from $58$ English-speaking celebrities and politicians via online video sharing platforms, such as YouTube.
The authors took special care to match the speaking style for each pair of spoofed and authentic instances to prevent the model from learning to distinguish spoofs based on extraneous characteristics (i.e., ``shortcuts''), such as speaking style, background noise, or setting.
For instance, for a spoofed speech by Barack Obama, an authentic speech was also included.
Our objective is for the model to distinguish spoofed audio based on either disfluencies that indicate poor naturalness or artifacts resulting from the text-to-speech (TTS) process.

% Because we are mainly interested in real-world model performance on unseen audio recordings, we train our models on the ASVspoof dataset (all splits) and use the ``In-the-Wild'' dataset to evaluate the models' generalization capabilities.
Since our primary concern is the real-world performance of the models on unseen audio recordings, we train them on the entire ASVspoof dataset (all splits) and assess their generalization abilities using the "In-the-Wild" dataset.
% We are following prior research and train our models on the ``train'' and ``dev'' partitions of ASVspoof.
% However, prior research has demonstrated that assessing the real-world generalization capacity of a model utilizing ASVspoof test data has limitations~\cite{muller2022does}.
% Therefore, we employ the ``In-the-Wild'' dataset to evaluate our models.

% We use two datasets for our experiments:
% The ASVspoof 2019 dataset (the \emph{Logical Access} (LA) section)~\cite{todisco2019asvspoof}, which is one of the most established anti-spoofing datasets, used by virtually all related work
% ~\cite{tak2021end,tak2021EndtoEnd,ge2021raw,wang2021Comparative,lavrentyeva_audio_2017,lavrentyeva_stc_2019,afchar2018MesoNet,vaswani2017attention}.
% This dataset comprises audio files that are either real (authentic recordings of human speech) or fake (synthesized or manipulated audio). 
% The synthetic audio files are generated using 19 distinct TTS synthesis algorithms, which are considered a threat to the authenticity of the human voice in terms of spoofing detection, and are hence labelled as `attacks' by ASVspoof. 
% The dataset contains 19 attackers, designated as A1 to A19, and for each attacker, there are 4914 synthetic audio recordings and 7355 real samples.

% Additionally, we use the ``In-the-Wild''~\cite{muller2022does} dataset, which features
% $37.9$ hours of audio clips that are either fake ($17.2$ hours) or real ($20.7$ hours).
% This audio comes from $58$ English-speaking celebrities and politicians, collected from Online Video Sharing Platforms such as YouTube. 
% Special care has been taken by the authors to match the speaking style for the pairs of spoofed and bona-fide instances.
% For example, for a spoofed speech of barack obama, an authentic one has been included.
% The motivation is that the model does not learn to discriminate spoofs on unwanted features (i.e. 'shortcuts'), for example, style of speaking, setting, or background ambient noise.

% Following related work, we are training on the ``train'' and ``dev'' split of ASVspoof.
% However, related work has shown that evaluating the real-world generalization capability of a model using ASVspoof test data has limitations.
% That is why we use the ``In-the-Wild'' dataset to evaluate our models.

% We use two datasets for our experiments:
% First, the ASVspoof 2019 dataset~\cite{todisco2019asvspoof}, specifically the \emph{Logical Access} (LA) section, which we use for model training.
% % We use the ASVspoof 2019 dataset~\cite{todisco2019asvspoof} to train %and evaluate 
% % our models, specifically the \emph{Logical Access} (LA) section. 
% This dataset comprises audio files that are either real (authentic recordings of human speech) or fake (synthesized or manipulated audio). 
% The synthetic audio files are generated using 19 distinct TTS synthesis algorithms, which are considered a threat to the authenticity of the human voice in terms of spoofing detection, and are hence labelled as `attacks' by ASVspoof. 
% The dataset contains 19 attackers, designated as A1 to A19, and for each attacker, there are 4914 synthetic audio recordings and 7355 real samples. 
% All audio files are resampled to $16kHz$.
% We train on the ``train'' and ``dev'' split, thereby following related work 
% \cite{tak2021end,tak2021EndtoEnd,ge2021raw,wang2021Comparative,lavrentyeva_audio_2017,lavrentyeva_stc_2019,afchar2018MesoNet,vaswani2017attention}.

% Related work has shown that evaluating the real-world generalization capability of a model using ASVspoof test data has limitations.
% Thus, we use the ``In-the-Wild'' dataset for model generalisation, which features
% $37.9$ hours of audio clips that are either fake ($17.2$ hours) or real ($20.7$ hours).
% This audio comes from English-speaking celebrities and politicians, both from present and past.
% The fake clips are created by segmenting $219$ of publicly available video and audio files  from Online Video Sharing Platforms that explicitly advertise audio deepfakes.

%and evaluate on the ``eval'' portion of the data, which features unseen speakers and attacks.
% This dataset is widely recognized as the most prominent audio deefake dataset and is employed by virtually all related research
% ~\cite{tak2021end,tak2021EndtoEnd,ge2021raw,wang2021Comparative,lavrentyeva_audio_2017,lavrentyeva_stc_2019,afchar2018MesoNet,vaswani2017attention}.


\begin{table*}[h!]
    \centering
    % \resizebox{0.48\textwidth}{!}{%
    \input{res/results}
    % }
    \caption{Model evaluation results on the ``In-the-Wild'' dataset. The results are averaged over three independent runs, with the standard deviation displayed.}
    \label{tab:res}
\end{table*}

\subsection{Data-augmentation and Hyperparameters}
Previous research has identified a significant learning shortcut in the ASVspoof 2019 dataset, whereby the duration of silence in an audio file is highly correlated with its corresponding label. This correlation has led to an overestimation of anti-spoofing system performance~\cite{muller2021Speech}. To obtain a realistic estimate of the anti-spoofing model performance, it is crucial to eliminate this shortcut. 
We address this issue by following the suggestions made by related work~\cite{muller2021Speech, zhang122021effect} and trim the beginning and end silences of an audio file. Moreover, we randomly select a 2-second segment from the remaining audio to ensure that all audio files have equal length. This prevents our models from using the presence or position of the cut-off as a new learning shortcut. We apply this technique to all subsequent analyses.

In addition, inspired by the widespread use of data augmentation in the image domain, we employ the following audio data augmentations in all subsequent analyses. By doing so, we further aim to avoid shortcuts, model overfitting, and promote model generalization.
% \begin{itemize}
%     \itemsep0em
%     \item Adversarial Retraining~\cite{goodfellow2014explaining}: We use the Fast Gradient Sign Method (FGSM) to craft adversarial examples with a probability of $25\%$ and a magnitude of $0.25\%$ of the input magnitude.
%     This approach has been shown to increase model generalization~\cite{goodfellow2014explaining} and regularisation~\cite{Regulari30:online}.
%     \item Audio Augmentations~\cite{iver56au88:online}.
%     We use room impulse response, frequency masking, pitch- and timeshift, gain, high, low- and bandpass filters, polarity inversion and clipping to diversify the input data (probability $60\%$).
%     \item Compression. We use MP3, ulaw and alaw codecs to partially encode the input (probability $20\%$)
%     \item We use the MusDB18~\cite{musdb18} and Noise ESC 50~\cite{piczak2015dataset} datasets to add random clips of noise and music to the audio files (probability $5\%$).
% \end{itemize}

First, we use Adversarial Retraining~\cite{goodfellow2014explaining}. Namely, we employ the Fast Gradient Sign Method (FGSM) to craft adversarial examples with a probability of $25\%$ and a magnitude of $0.25\%$ of the input magnitude and supply these as additional training examples. This method has been shown to improve model generalization~\cite{goodfellow2014explaining} and regularization~\cite{Regulari30:online}.
Second, we use audio augmentations~\cite{iver56au88:online} such as room impulse response, frequency masking, pitch- and timeshift, gain, high, low- and bandpass filters, polarity inversion, and clipping to diversify the input data with a probability of $60\%$.
Third, with a probability of $20\%$, we partially encode the input using MP3, ulaw, and alaw codecs to perform compression.
Lastly, we add random clips of noise and music to the audio files with a probability of $5\%$ by utilizing the MusDB18~\cite{musdb18} and Noise ESC 50~\cite{piczak2015dataset} datasets.

We utilize the Adam optimizer with a learning rate of $5 \cdot 10^{-3}$ to train all models. The models are trained for $25$ epochs with a weight decay of $10^{-6}$ and a batch-size of $32$.
To prevent overfitting, we employ early stopping with a patience of $3$ epochs and a minimum delta of $5 \cdot 10^{-4}$. We implement the models using Python and PyTorch.
For the Constant-Q Transform (CQT), we use a window size of $128$ samples and a hop size of $64$ samples with the ``Hann'' windowing function.
% In \cref{eq:logscale}, we set $c=+3$ because $\max \text{log}_e(Z_Q) < 3$.
We train all models using an Nvidia DGX-A100 server, which is equipped with eight A100 GPUs, each having a memory of 40GB, and a total server memory of 1024GB. It features two AMD Rome 7742 processors, each with 64 cores.

% \todo[inline]{Say STFT parameters}
% \todo[inline]{Say we use python + pytorch}

\subsection{Evaluation and Results}




% Following related work~\cite{todisco2019asvspoof, nautsch2021ASVspoof,tak2021EndtoEnd,tak2021end,ge2021raw}, we evaluate our model using the Equal Error Rate (EER), which is the location on a ROC or DET curve where the false acceptance rate and false rejection rate are equal.
% For each configuration, we repeat three independent trials and report the mean and standard-deviation.
% \Cref{tab:res} presents the results for our proposed model, and models from related work:
% RawNet2~\cite{tak2021EndtoEnd} and RawGatST~\cite{tak2021end}, which process ``raw'' audio directly, and the LCNN model~\cite{wang2021Comparative}, which uses magnitude-based CQT features.
% We observe the following:
% First, the complex-valued model is able to outperform related work by about $3\%$ EER absolute.
% Second, we observe the least amount of overfitting, as indicated by the gap between train and test performance.

We adopt the Equal Error Rate (EER) as the performance metric for our model evaluation, consistent with previous studies~\cite{tak2021end,tak2021EndtoEnd,ge2021raw,todisco2019asvspoof,nautsch2021ASVspoof}. 
EER is the point on the Receiver Operating Characteristic (ROC) curve where the false acceptance rate and false rejection rate are equal. 
For each experimental configuration, we conduct three independent trials and report the mean and standard deviation of the EER. 
\Cref{tab:res} summarizes the results of our proposed model compared to models from related work.
We observe the following: Firstly, our complex-valued model demonstrates an absolute improvement over related work by about $3\%$ EER when compared to ``raw'' features and $10\%$ EER when using magnitude-based CQT features. Secondly, we observe the least amount of overfitting, as indicated by the small gap between the training and testing performance.

\subsection{Ablation Study}
In order to evaluate the impact of the phase information, we perform an ablation study where we keep all parameters for our proposed model, but discard or randomize the phase information from the complex spectrogram.
\Cref{tab:abl} presents the results.
We observe that the removal of phase information ("zero phase") results in a $4\%$ degradation in model performance with respect to EER. This suggests that the proposed model has indeed learned to detect spoofing attacks by utilizing the mismatch between phase and magnitude information to some extent.
Furthermore, randomizing the phase information causes an additional $4\%$ decrease in performance with respect to EER. We presume that this is due to the fact that the model not only lacks phase information, but also has to cope with a significant amount of noise when dealing with randomly generated phase information.

\begin{table}[]
    \centering
    \resizebox{0.48\textwidth}{!}{%
    \input{res/ablation}
    }
    \caption{Ablation study results for the C-CQT feature: full phase retention, random phase selection, or zero assignment.}
    \label{tab:abl}
\end{table}

\subsection{Explainable AI}

\begin{figure}
    \centering
    % \begin{subfigure}[b]{0.49\textwidth}
        %\includegraphics[width=0.99\textwidth]{res/xai_128_0.png}
        % \includegraphics[trim={19cm 1.5cm 7cm 4cm},clip,width=0.49\textwidth]{res/ccqcc_log_log_sg_0.png}
        % \caption{Bona-fide instance.}
    % \end{subfigure}
    % \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[trim={19cm 1.5cm 10cm 4cm},clip,width=0.45\textwidth]{res/ccqcc_log_log_sg_1.png}
    %     %\includegraphics[width=0.99\textwidth]{res/xai_128_1.png}
    %     \caption{Spoofed instance.}
    % \end{subfigure}
    \caption{SmoothGrad~\cite{smilkov2017smoothgrad} applied on a spoofed instance from the ASVspoof dataset.
    %The resulting XAI output (red) is overlaid on the C-CQT feature (greyscale).
    %Top: Bona-fide instance. 
    %Bottom: Spoofed instance. Discriminative information is contained in the upper frequency bands.
    }
    \label{fig:xai}
\end{figure}

Our model allows the application of explainable AI techniques such as saliency maps~\cite{simonyan2014very} and Smooth Grad~\cite{smilkov2017smoothgrad}. These techniques allow us to visualize how our model processes audio in the frequency domain, thereby enabling us to gain insight into the decision-making process of our model.
To demonstrate the effectiveness of these techniques, we apply Smooth Grad 
%to both bona-fide and spoofed audio instances, 
and present an exemplary output in \Cref{fig:xai}. Our analysis shows that the model does not rely on any obvious shortcuts, such as the duration of silence\cite{muller2021Speech} or other artifacts such as sampling or ringing issues in the upper frequency bands. Instead, the model focuses on the speech signal itself, as evidenced by the red XAI-overlay coinciding with the spectro-temporal bins containing descriptive features.


\section{Conclusion and Future Work}
This paper introduces a novel approach to voice anti-spoofing, which involves utilizing complex-valued features and complex-valued neural networks. This approach is motivated by the fact that magnitude-based feature extraction discards phase information, which is difficult to spoof yet crucial for producing natural-sounding synthesized speech, thereby constituting a useful input feature to voice anti-spoofing systems.
Building on previous research, we thus propose using the complex-valued Constant-Q Transform (C-CQT) as a new input feature and suggest a corresponding complex-valued neural architecture. 
Our proposed approach not only outperforms previous related work but also allows for explainability through established XAI-methods, which is lacking in ``raw''-feature-based models.
Through ablation studies, we demonstrate that our model has effectively learned to use phase information to distinguish between spoofed and bona-fide audio. These results indicate the potential of our approach in improving the accuracy of voice anti-spoofing and advancing the understanding of the underlying decision-making process.

% However, we believe that there is still room for improvement in our proposed neural architecture. Although the current model is simple, it already outperforms related work that consists of more advanced components. We think that further refinement of our architecture could lead to even better performance in detecting spoofed voice signals.

% %Alternativvorschlag
% In summary, we propose a well-performing architecture useful for anti-spoofing.
% Even though our current model is simple, it already outperforms related work that consists of more advanced components. 
% Thanks to the fully neuronal architecture of our approach, we believe that further refinements are easy to integrate and might lead to even better performance in detecting spoofed voice signals. 

In summary, we suggest an effective architecture that can be useful for anti-spoofing purposes. Despite the simplicity of our current model, it already surpasses the performance of related works that employ more sophisticated components. We are confident that incorporating further model refinements would be straightforward and could potentially enhance the ability to detect spoofed voice signals.
